Attributable-Watermarking of Speech Generative Models

Generative models are now capable of synthesizing images, speeches, and videos that are hardly distinguishable from authentic contents. Such capabilities cause concerns such as malicious impersonation and IP theft. This paper investigates a solution for model attribution, i.e., the classification of synthetic contents by their source models via watermarks embedded in the contents. Building on past success of model attribution in the image domain, we discuss algorithmic improvements for generating user-end speech models that empirically achieve high attribution accuracy, while maintaining high generation quality. We show the trade off between attributability and generation quality under a variety of attacks on generated speech signals attempting to remove the watermarks, and the feasibility of learning robust watermarks against these attacks.

==> backup.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% File:     spconf.sty          (LaTeX Document style option "spconf")
%
% Usage:    \documentclass{article}
%           \usepackage{spconf}
%
%           Or for LaTeX 2.09:
% Usage:    \documentstyle[...,spconf,...]{article}
%
% Purpose:
%
% Style file for Signal Processing Society Conferences (ICASSP, ICIP).
% Features:
%    - correct page size (175mm x 226mm)
%    - twocolumn format
%    - boldfaced, numbered, and centered section headings
%    - correct subsection and subsubsection headings
%    - use \title{xx} for title, will be typeset all uppercase
%    - use \name{xx} for author name(s) only, will be typeset in italics
%    - use \address{xx} for one address of all authors
%    - use \twoauthors{author1}{address1}{author2}{address2}
%         for two (or more) authors with two separate addresses
%    - note: no need for \author nor \date
%    - optional: can use \thanks{xx} within \name or \twoauthors,
%         asterisk is not printed after name nor in footnote
%    - optional: can use \sthanks{xx} after each name within \name or
%         \twoauthors if different thanks for each author,
%         footnote symbol will appear for each name and footnote
%    - optional: use \ninept to typeset text in 9 pt; default is 10pt.
%
% Example of use for one or more authors at a common address and
%    common support. For distinct support acknowledgments,
%    use \sthanks{xx} after each name.
%
%                 \documentclass{article}
%                 \usepackage{spconf}
%                 \title{Title of the paper}
%                 \name{George P. Burdell and John Q. Professor
%                       \thanks{This work was supported by...}}
%                 \address{Common address, department \\
%                          City, etc \\
%                          optional e-mail address}
%
%                 \begin{document}
%  OPTIONAL -->   \ninept            <-- OPTIONAL, for nine pt only
%                 \maketitle
%                 \begin{abstract}
%                 This is the abstract for my paper.
%                 \end{abstract}
%                         .
%                 Insert text of paper
%                         .
%                 \end{document}
%
% Example of use for two authors at two distinct addresses with only
%    one support acknowledgment. For distinct support acknowledgments,
%    use \sthanks{xx} after each name.
%
%                 \documentclass{article}
%                 \usepackage{spconf}
%                 \title{Title of the paper}
%                 \twoauthors{John Doe
%                       \thanks{This work was supported by...}}
%                            {Doe's address, department \\
%                             City, etc \\
%                             optional e-mail address}
%                            {Judy Smith}
%                            {Smith's address, department \\
%                             City, etc \\
%                             optional e-mail address}
%
%                 \begin{document}
%  OPTIONAL -->   \ninept            <-- OPTIONAL, for nine pt only
%                 \maketitle
%                 \begin{abstract}
%                 This is the abstract for my paper.
%                 \end{abstract}
%                         .
%                 Insert text of paper
%                         .
%                 \end{document}
%
% Preprint Option (Only for preprints, not for submissions!):
%    - can create a preprint titlepage footer by using the
%         "preprint" option with the \usepackage{spconf} command
%    - use \copyrightnotice{\copyright xx} for copyright information
%    - use \toappear{To appear in xx} for publication name
% Example of preprint use:
%
%                 \documentclass{article}
%                 \usepackage[preprint]{spconf}
%                         .
%                 \copyrightnotice{\copyright\ IEEE 2000}
%                 \toappear{To appear in {\it Proc.\ ICASSP2000,
%                    June 05-09, 2000, Istanbul, Turkey}}
%
%
% PLEASE REPORT ANY BUGS
%
% Author:  Stephen Martucci  -- stephen.martucci@ieee.org
%
% Date:    3 May 2000
%
% Updated: Lance Cotton, Ulf-Dietrich Braumann, 11 May 2006
% Change:  Added keywords/Index Terms section
% Change:  Added \emergencystretch=11pt, Lance Cotton, 26-Sept-2007
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% These commands change default text fonts to the scalable PostScript
% fonts Times, Helvetica, and Courier. However, they do not change
% the default math fonts. After conversion to PDF, text will look good
% at any scale but math symbols and equations may not.
% If instead you use the PostScript Type 1 implementation of the
% Computer Modern fonts from the American Mathematical Society, which
% will make all fonts (text and math) scalable, comment out the
% following three lines. Those fonts use the same metrics as the Knuth
% Computer Modern fonts and therefore no font redefinition is needed.
\renewcommand{\sfdefault}{phv}
\renewcommand{\rmdefault}{ptm}
\renewcommand{\ttdefault}{pcr}

%\oddsidemargin  -0.31in
%\evensidemargin -0.31in
\oddsidemargin  -6.2truemm
\evensidemargin -6.2truemm

\topmargin 0truept
\headheight 0truept
\headsep 0truept
%\footheight 0truept
%\footskip 0truept
\textheight 229truemm
\textwidth 178truemm

\twocolumn
\columnsep 6truemm
\pagestyle{empty}

\emergencystretch=11pt

\def\ninept{\def\baselinestretch{.95}\let\normalsize\small\normalsize}

\def\maketitle{\par
 \begingroup
 \def\thefootnote{}
 \def\@makefnmark{\hbox
 {$^{\@thefnmark}$\hss}}
 \if@twocolumn
 \twocolumn[\@maketitle]
 \else \newpage
 \global\@topnum\z@ \@maketitle \fi\@thanks
 \endgroup
 \setcounter{footnote}{0}
 \let\maketitle\relax
 \let\@maketitle\relax
 \gdef\thefootnote{\arabic{footnote}}\gdef\@@savethanks{}%
 \gdef\@thanks{}\gdef\@author{}\gdef\@title{}\let\thanks\relax}

\def\@maketitle{\newpage
 \null
 \vskip 2em \begin{center}
 {\large \bf \@title \par} \vskip 1.5em {\large \lineskip .5em
\begin{tabular}[t]{c}\@name \\ \@address
 \end{tabular}\par} \end{center}
 \par
 \vskip 1.5em}

\def\title#1{\gdef\@title{\uppercase{#1}}}
\def\name#1{\gdef\@name{{\em #1}\\}}
\def\address#1{\gdef\@address{#1}}
\gdef\@title{\uppercase{title of paper}}
\gdef\@name{{\em Name of author}\\}
\gdef\@address{Address - Line 1 \\
               Address - Line 2 \\
               Address - Line 3}

\let\@@savethanks\thanks
\def\thanks#1{\gdef\thefootnote{}\@@savethanks{#1}}
\def\sthanks#1{\gdef\thefootnote{\fnsymbol{footnote}}\@@savethanks{#1}}

\def\twoauthors#1#2#3#4{\gdef\@address{}
   \gdef\@name{\begin{tabular}{@{}c@{}}
        {\em #1} \\ \\
        #2\relax
   \end{tabular}\hskip 1in\begin{tabular}{@{}c@{}}
        {\em #3} \\ \\
        #4\relax
\end{tabular}}}

\def\@sect#1#2#3#4#5#6[#7]#8{
   \refstepcounter{#1}\edef\@svsec{\csname the#1\endcsname.\hskip 0.6em}
       \begingroup \ifnum #2=1\bf\centering
          {\interlinepenalty \@M
             \@svsec\uppercase{#8}\par}\else\ifnum #2=2\bf
          \noindent{\interlinepenalty \@M \@svsec #8\par}\else\it
          \noindent{\interlinepenalty \@M
             \@svsec #8\par}\fi\fi\endgroup
       \csname #1mark\endcsname{#7}\addcontentsline
         {toc}{#1}{\protect\numberline{\csname the#1\endcsname} #7}
     \@tempskipa #5\relax
     \@xsect{\@tempskipa}}

\def\abstract{\begin{center}
{\bf ABSTRACT\vspace{-.5em}\vspace{0pt}}
\end{center}}
\def\endabstract{\par}

% Keyword section, added by Lance Cotton, adapted from IEEEtrans, corrected by Ulf-Dietrich Braumann
\def\keywords{\vspace{.5em}
{\bfseries\textit{Index Terms}---\,\relax%
}}
\def\endkeywords{\par} 

\def\copyrightnotice#1{\gdef\@copyrightnotice{#1}}
\let\@copyrightnotice\relax
\def\toappear#1{\gdef\@toappear{#1}}\let\@toappear\relax

\newif\if@preprint\@preprintfalse
\@namedef{ds@preprint}{\global\@preprinttrue}
\@options
\def\ps@preprint{\def\mypage{}\let\@mkboth\@gobbletwo\def\@oddhead{}
  \def\@oddfoot{\rlap{\@toappear}\hfil\mypage\hfil
    \llap{\@copyrightnotice}
    \gdef\mypage{\thepage}\gdef\@toappear{}\gdef\@copyrightnotice{}}}

\if@preprint\ps@preprint
\else\ps@empty\flushbottom\fi

\def\thebibliography#1{\section{References}\list
 {[\arabic{enumi}]}{\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
 \advance\leftmargin\labelsep
 \usecounter{enumi}}
 \def\newblock{\hskip .11em plus .33em minus .07em}
 \sloppy\clubpenalty4000\widowpenalty4000
 \sfcode`\.=1000\relax}
\let\endthebibliography=\endlist

\long\def\@makecaption#1#2{
 \vskip 10pt
 \setbox\@tempboxa\hbox{#1. #2}
 \ifdim \wd\@tempboxa >\hsize #1. #2\par \else \hbox
to\hsize{\hfil\box\@tempboxa\hfil}
 \fi}

\def\fnum@figure{{\bf Fig.\ \thefigure}}
\def\fnum@table{{\bf Table \thetable}}

\flushbottom

%%%% EOF
